A Comprehensive Survey of Threshold Signatures: NIST Standards, Post-Quantum Cryptography, Exotic Techniques, and Real-World Applications

Threshold digital signatures enable a distributed execution of signature functionalities and will play a crucial role in the security of emerging decentralized next-generation networked systems and applications. In this paper, we provide a comprehensive and systematic survey of threshold and distributed signatures with advanced features. Our survey encompasses threshold signatures in conventional and post-quantum cryptography (PQC) settings and captures custom-design and standard signatures (e.g., conventional NIST and NIST-PQC). We examine both generic (via secure multi-party computation) and custom thresholding techniques for a myriad of signature families while investigating exotic signatures, real-life applications, and potential future research direction.

==> bodies/performance_metrics.tex <==
\subsubsection{Performance Metrics of Threshold Digital Signatures}
\label{sec:PerMetDigSig}
The performance metrics for threshold digital signatures have been outlined by NIST in their latest document titled "\textit{NIST First Call for Multi-Party Threshold Schemes}" \cite{brandao2023nist}. The metrics are as follows:

\begin{itemize}
\item \textit{Memory overhead}. Demonstrates the total storage required and can be affected by signature and key sizes.
\item \textit{Processing time}. Shows the amount of time for signature generation and can be affected by signature algorithms.
\item \textit{Communication overhead}. Denotes the amount of data communicated through the network and can be affected by signature and key sizes. 
\item \textit{Networking time}. Demonstrates the networking delay. % Signature and key sizes can affect this metric.
\item \textit{Round complexity}. Demonstrates the number of alterations in the direction of communicated messages. 
\item \textit{End-to-end delay}: Indicates the total delay affected by processing time, networking time, and round complexity.
\item \textit{Threshold parameters}:
Changing the parameter $t$ in a $(t,n)$ threshold digital signature has implications for the security properties of \textit{Confidentiality} and \textit{Availability} in a way that, while improving one, degrades another. Increasing the value of $t$ improves confidentiality by increasing the number of parties required to generate a signature (e.g., $\mathit{t=n}$), but it compromises availability if any party refuses to participate in recovering the secrets. Conversely, decreasing the value of $t$ enhances availability but reduces the chance of achieving high confidentiality since fewer parties are required to collude and generate a signature if some parties are malicious.
\end{itemize}



==> commands.tex <==
\newcommand{\adversary}{\mathcal{A}}


==> notes.tex <==



ECDSA CDH in the table -> make it define above 




**************
Comparison of scheme in table ?? Description of comparison ?
Should n=24 be n = 24 ? I made it to the first
Should reference SIS and LWE everywhere





SSS:
Space around = in SSS definition
definition of SSS does not have t in itself




MPC:
Have I mentioned ROM ?
Have I mentioned ZKP ?
UC in MPC ?





Performance:
Performance metrics specific to threshold only? Should I mention sth.
Performance not visible



Group/Ring/Multi:
Ring prime order
Ma et al. \cite{} proposed an efficient multi-signature scheme based on the DL assumption that is secure in the plain model. Compared to the scheme \cite{bellare2006multi}, this scheme requires one less signing round with the number of exponentiations same in signing and verifying. Compared to \cite{bagherzandi2008multisignatures}, it requires the same number of exponentiations in the signing and verifying procedures, but the signing rounds is one round of interaction less.
Threshold Group ..... yavuz new scheme
group table: delerablee2006dynamic full anonmity define down not above



PQC:
2014 scheme: italic for hash and sign ?
Dan boneh performance



** Section 8,2 -> vspace
** Section 5 -> vpsace
** Section 4.0.2 -> vpsace
